Exposing the Functionalities of Neurons for Gated Recurrent Unit Based Sequence-to-Sequence Model

The goal of this paper is to report certain scientific discoveries about a Seq2Seq model. It is known that analyzing the behavior of RNN-based models at the neuron level is considered a more challenging task than analyzing a DNN or CNN models due to their recursive mechanism in nature. This paper aims to provide neuron-level analysis to explain why a vanilla GRU-based Seq2Seq model without attention can achieve token-positioning. We found four different types of neurons: storing, counting, triggering, and outputting and further uncover the mechanism for these neurons to work together in order to produce the right token in the right position.

==> sections/backup-section5-findings.tex <==

\section{Summary of Findings}

%Firstly, we explain the mechanism of 4 functional neurons found in Seq2Seq model,  including \emph{storing}, \emph{counting}, \emph{triggering} and \emph{outputting}, to provide an overview about our findings as well as the hypothesis on how they interact to make Seq2Seq output the right token at the right time-step. Experiment details are discussed in Section X to confirm our hypothesis.

For each token, model has its own four neuron sets to help to keep the necessary information and output the token at the right position. There may exist overlap on each neuron sets since neurons can be multi-functional. %After realizing the function of four neuron sets, following the hypothesis, we can answer all the research questions mentioned in Section X to yield a better understanding on Seq2Seq model. 
Figure \ref{flow_chart} is the conceptual graph which shows when do those important neuron sets exist and how they affect each others.

\begin{figure*}%[h]
  \centering
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \includegraphics[width=0.9\textwidth]{figures/NeuronInteraction.png}
  \caption{The whole inference process of token positioning task and the neuron interaction. With the interaction of the four types of neurons, we are capable of answering all the research questions mentioned in Section 1.}
  %\label{flow_chart}
\end{figure*}

\textbf{Storing Neurons}  
For each token, there is a small set ($15\% \sim 25\%$) of neurons, defined as $S_{store,tok}$, that jointly \emph{storing} token information. $S_{store,tok}$ is shared among each token with different positions, and they are established during the encoder stage when the token is provided. $S_{store,tok}$ remains largely unchanged until $h_{t=T-1}$, one step before the assigned position is reached in the decoder.

%Storing the information about the specified token. This type of neurons are eager to activate \emph{outputting neurons} before the specified time-step but block by the gate inside the Seq2Seq model.


\textbf{Counting Neurons} For each token, there is a small set (about $20\%$) of neurons, defined as $S_{cd,tok}$, whose values keep increasing, or decreasing, with $t$ from t = 0 to T - 2, and eventually reaches the maximum/minimum to activate $S_{trig,tok}$ at $t = T-1$.
Therefore, it can indicate how many time step are left wo output the specified token.

%Indicating how many time-step left to output the specified token. Note that we found the counting information is not stored as real values, instead they jointly behave as a incremental function that gradually reaches the optimal value before specified time-step.

 %$S_{cd,tok}$ is also invariant with positions and act as a kind of counter. %They reach the highest values, usually $>0.75$ or $<-0.75$, 
%At $t = T - 2$, the counting neuron reaches the optimal value to activate $S_{trig,tok}$.

\textbf{Triggering Neurons} 
For each token (regardless of the position), there is a small set ($15\% \sim 25\%$) of neurons, defined as $S_{trig,tok}$, that would become activated by counting neuron at $t = T-1$. Those neurons are responsible to control when the storing neuron can affect the outputting neuron. As a result, the model can output the assigned token at exactly the next time step when $S_{trig,tok}$ is activated at $T-1$. 

%After \emph{counting neurons} reach optimal value, the \emph{trigger neurons} will be activated. These neurons unblock the \emph{storing neurons} by changing the gate state to enable \emph{storing neurons} the ability to affect the \emph{outputting neurons} to cause model output the specified token.

\textbf{Outputting Neurons} For each token, there is a small set of neurons (about $20\%$) which cause the fully connected layer to output the target token. At $t$ = $T$, $S_{store,tok}$ influences the model through h gate, and $S_{trig,tok}$ influences the model by z and r gate, to activate the $S_{out,tok}$ to its extreme value. Next, since $S_{fc,tok}$ is connected to the larger weights of tokens with the assigned token, the probability of this token increases at $t = T$.

%Neurons that directly contribute to the token probability after the decoder output layer and cause the model output the specified token.

%For each token, it has its own four neuron sets and there may exist overlap on each neuron sets since neurons can be multi-functional. After realizing the function of four neuron sets, following the hypothesis, we can answer all the research questions mentioned in Section X to yield a better understanding on Seq2Seq model.

\textbf{Length-control and rhyme-control tasks}
Following shows that the other two sub-tasks, length-control and rhyme-control, can achieve similar training performance and analyzing results as the main task we discuss in section 4. When the target token is always set to "EOS", the model can learn to control the length of the output. Using the same data set, model structure and training process mentioned in Section 2, the accuracy reaches 99.xx. The analysis results are also similar as we record in Appendix C. The rhyme-control task also has similar situation with training accuracy = xx, except we change the assigned token to a specific rhyme. The rhyme dataset can generated as following: get the rhyme of the last word in the output  as "token" and get the length of the output as "position". 

\begin{comment}
\subsection{Related Tasks}

Following shows that the other two sub-tasks can achieve similar training performance and analyzing results as the main task we discuss in section 4.

\textbf{Length-control task: Always set token to "EOS".} 
When the target token is always set to "EOS", the model can learn to control the length of output sequence. Using this dataset with the same model structure and training process as mentioned in section 2, the accuracy reaches 99.xx. In addition, with the similar analysis steps in section 3 and 4, one can also find out the counting neurons and output neurons. The related figures and accuracy is at Appendix C. 
    
\textbf{Rhyme-control task: Set token corresponds to a cluster of word in the dictionary.}
    In lyric or poem generation, it requires the output sequence to end with a word with a specific rhyme. For this task, one can generate the training dataset by two steps: (1) Get the rhyme of the last word in the output sequence as "token". (2) Get the length of the output sequence as "position". Then concatenate these two control signals to the input sequence, as the example in the section 1. And in the inference process, concatenate arbitrary "rhyme" and "length" to any sequence to get the correct rhyme. In our dataset, we have 35 rhyme tokens and the model can get accuracy to xx. Following the similar analysis steps, we can also find out the important neuron sets such as storing neuron (of each rhyme) and the counting neurons as in Appendix C.


\end{comment}


%\textbf{Hypothesis} Summarize the neuron interaction to answer the research questions. [Add Later]

% Therefore, the inference procedure can be summarized as :
% \begin{enumerate}
%     \item Encoding the \emph{token information} in the \emph{storing neuron}
%     \item Encoding the \emph{position information} in the \emph{counting neuron}
%     \item \emph{Counting neuron} activate \emph{triggering neuron}.
%     \item \emph{Triggering neuron} activate \emph{outputting neuron} to output specified token.
% \end{enumerate}
% With the interaction of the four types of neurons, we are capable of answering all the research questions mentioned in Section 1.

==> sections/ck20jimmy_Gate_Interaction.tex <==
% \section{Appendix}
\section{Interaction between Functional Neurons and Gates inside GRU}
After realizing the validity of four functional neurons, we go deep into the formulation of GRU, including each gate and its corresponding weight.
% After the model encoded the word information with storing neuron and the position information with counting neuron, it raised another question to  solve: what is the interaction between storing and counting neuron to trigger model output the right word at the right time-step ? 
In this section, we combine the mathematical and the empirical perspective to investigate the relationship between functional neurons and gates. In Fig. X, we visualize the neuron interaction  to clarify our argument. 

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/appendix_trig_vis.png}
    \caption{Visualization of neurons interaction. }
    \label{gruv-1}
\end{figure}

%\newpage

Recall the mathematical formulation of GRU cell:

% \begin{small}
\begin{equation*}
% \begin{aligned}
GRU\begin{cases}
    &z_t = \sigma(W_{z}x_t + U_{z}h_{t-1} + b_z)  \\
    &r_t = \sigma(W_{r}x_t + U_{r}h_{t-1} + b_r) \\
    &\widetilde{h_t} = \text{tanh}(W_{h}x_t + U_{h}(r_t \odot h_{t-1}) + b_h)  \\ 
    &h_t = z_t \odot h_{t-1} + (1 - z_t) \odot \widetilde{h}_t\\
    \end{cases} \quad
GRU^{'}\begin{cases}
    &z_t = \sigma(U_{z}h_{t-1} + b_z)  \\
    &r_t = \sigma(U_{r}h_{t-1} + b_r) \\
    &\widetilde{h_t} = \text{tanh}(U_{h}(r_t \odot h_{t-1}) + b_h)  \\ 
    &h_t = z_t \odot h_{t-1} + (1 - z_t) \odot \widetilde{h}_t
    \end{cases}
% \begin{aligned}
%     &z_t = \sigma(W_{z}x_t + U_{z}h_{t-1} + b_z)  \\
%     &r_t = \sigma(W_{r}x_t + U_{r}h_{t-1} + b_r) \\
%     &\widetilde{h_t} = \text{tanh}(W_{h}x_t + U_{h}(r_t \odot h_{t-1}) + b_h)  \\ 
%     &h_t = z_t \odot h_{t-1} + (1 - z_t) \odot \widetilde{h}_t\\
% \end{aligned}
\label{GRU_Formula}
\end{equation*}
% \end{small}
% \caption{The original formulation of GRU and its simplified version}


with $z_t, r_t, h_t, \widetilde{h}_t$ as the \emph{update gate}, \emph{reset gate}, \emph{activation}, and \emph{candidate activation}. Since the random replacement experiment shows that $x_t$ has very few influence on $z_t, r_t, h_t$ that can be neglected, we simplify the formulation of GRU cell and noted as $GRU^{'}$.

% \begin{small}
% \begin{equation}
% \begin{aligned}
%     &z_t = \sigma(U_{z}h_{t-1} + b_z)  \\
%     &r_t = \sigma(U_{r}h_{t-1} + b_r) \\
%     &\widetilde{h_t} = \text{tanh}(U_{h}(r_t \odot h_{t-1}) + b_h)  \\ 
%     &h_t = z_t \odot h_{t-1} + (1 - z_t) \odot \widetilde{h}_t
% \end{aligned}
% \label{GRU}
% \end{equation}
% \end{small}

Then we can simply view the operation inside the $\sigma(\cdot)$ function as a linear transformation of $h_{t-1}$ to $z_t, r_t$ or $h_t$. Therefore, the weight $U_z, U_r, U_h$ are indeed the feature importance. In order to verify our hypothesis that triggering neurons trigger the storing neurons to affect the outputting neurons, we take the transition weight in $U_z, U_r, U_h$ as the measure for the triggering capability to the specific storing neuron and outputting neurons. Following the formulation above, for \emph{z gate}, the transition weight from triggering neuron to outputting neurons should be low in order to update the neuron value in $h_{t-1}$ (in Fig. X(a)), and for the \emph{r gate}, the transition weight from trigger neuron to storing neuron should be high in order to make $h_{t-1}$ effective to $\widetilde{h_t}$  or it will be masked.(in Fig. X(b))  After the value in each gate are determined, the transition weight in $U_h$ should be extreme value in order to trigger the outputting neurons to reach extreme value as well.(in Fig. X(c)) Additionally, we apply integrated gradient to check the impact from triggering neuron to outputting neurons, which shows the same result as directly analyzing the inner operation of GRU cell. Statistics are listed in Figure X and Table X.





% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{ccccc}
% 		\toprule
% 		Neurons set & Z gate & R gate & H gate \\
% 		\midrule
% 		$h_{T-1, store}$ & 7.9E-3 & 7.3E-3 & 6.7E-3\\
% 		$h_{T-1, trig}$ & 1.3E-2 & 9.8E-3 & 1.6E-3 \\
% 		Whole $h_{T-1}$ & 4.0E-3 & 5.1E-3  & 2.4E-3\\
% 		\bottomrule
		
% 	\end{tabular}
	
% 	\caption{Different $S_{Imp}$ importance through different gates by calculating integrated gradient score. The first and second columns show that $h_{T-1, trig}$ is the most important through z and r gate, whereas the third column shows that $h_{T-1, store}$ is the most important through h gate.}
% 	\label{IG_score}
% \end{table}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/appendix_z_impact.png}
%   \caption{Impact of triggering neurons to decrease \emph{z gate} value of outputting neurons. X-axis are sixteen $S_{fc,tok}$ neurons. Y-axis represents the impact from $h_{T-1, trig}$ (blue bars) and other neurons (red bars). Most blue bars have obvious negative values and it implies that it is $h_{T-1, trig}$ to increase $z_{T, fc}$.}
%   \label{z_impact}
% \end{figure}




\begin{figure}[h]
    \begin{center}
    
    \begin{minipage}[b]{0.43\textwidth}
        \centering
        	\begin{tabular}{ccccc}
    		\toprule
    		Neurons set & Z gate & R gate & H gate \\
    		\midrule
    		$h_{T-1, store}$ & 7.9E-3 & 7.3E-3 & 6.7E-3\\
    		$h_{T-1, trig}$ & 1.3E-2 & 9.8E-3 & 1.6E-3 \\
    		Whole $h_{T-1}$ & 4.0E-3 & 5.1E-3  & 2.4E-3\\
    		\bottomrule
        		
        	\end{tabular}
        	
        	\caption{Different $S_{Imp}$ importance through different gates by calculating integrated gradient score. The first and second columns show that $h_{T-1, trig}$ is the most important through z and r gate, whereas the third column shows that $h_{T-1, store}$ is the most important through h gate.}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.53\textwidth}
         \centering
         \includegraphics[width=0.6\textwidth]{figures/appendix_z_impact.png}
          \caption{Impact of triggering neurons to decrease \emph{z gate} value of outputting neurons. X-axis are sixteen $S_{fc,tok}$ neurons. Y-axis represents the impact from $h_{T-1, trig}$ (blue bars) and other neurons (red bars). Most blue bars have obvious negative values and it implies that it is $h_{T-1, trig}$ to increase $z_{T, fc}$.}
          \label{z_impact}
        
    \end{minipage}%
    \end{center}
    
    \label{POS_10}
\end{figure}



==> sections/neurips-instruction.tex <==
\section{Submission of papers to NeurIPS 2020}

NeurIPS requires electronic submissions.  The electronic submission site is
\begin{center}
  \url{https://cmt3.research.microsoft.com/NeurIPS2020/}
\end{center}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers to be submitted to NeurIPS 2020 must be prepared according to the
instructions presented here. Papers may only be up to eight pages long,
including figures. Additional pages \emph{containing only a section on the broader impact, acknowledgments and/or cited references} are allowed. Papers that exceed eight pages of content will not be reviewed, or in any other way considered for
presentation at the conference.

The margins in 2020 are the same as those in 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2020.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.

The only supported style file for NeurIPS 2020 is \verb+neurips_2020.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.

The file \verb+neurips_2020.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2020+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2020}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.


\section*{Broader Impact}

Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
biases in the data. If authors believe this is not applicable to them, authors can simply state this.

Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare 
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

\section*{References}

References follow the acknowledgments. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
{\bf Note that the Reference section does not count towards the eight pages of content that are allowed.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.

==> sections/results-backup.tex <==
\begin{comment}

\section{Experiment results}\label{section4}

In this section, we describe how we apply the neuron identification strategy to identify these four neuron sets and answer the three research questions. Because each token has their own functional neurons, we conducted experiments on the 50 most common tokens, i.g. $i$, $the$, or $you$, (48\% of the sample) and also the most common position (75\% of the sample), from 1 to 13, on each dataset. The detailed accuracy are recorded in Appendix C. Also, we use $S_{store,A}$, $S_{count,A}$, $S_{trig,A}$, and, $S_{out,A}$ to indicate the storing, counting, triggering and outputting neurons for token A at hidden state t.

%We take the assigned token “A” and the position “T” as an example (output A at time step T). In addition, noting that every token in the dataset has their own important neuron set, %For example, token A use neurons {1, 3, 5} as its storing neuron while token B use neurons {2, 4, 6} as its storing neuron. 
%so executing three-steps strategy one time can only find out the important neurons for only one token. Therefore,  


\begin{figure*}
    \centering
    \includegraphics[width = 0.9\textwidth]{figures/pca_eating.png}
    \caption{PCA on $S_{store,tok}$ for ten common tokens from encoder to decoder. We select 500 sample for each common word with $T$ = 5 (5000 samples in total), and perform the same PCA transformation on their $S_{store}$. It implies that model remains token information unchanged from $t$ = \emph{Token} until triggering other neurons at $t$ = 4.}
    \label{fig:pca_word}
\end{figure*}

\subsection{How does the model store the $token$ information?}
The first step to answer this question is to find out the storing neurons. 
For every specified token A and position T, we label samples that "\emph{output A at position T}” as 0 and label samples that “\emph{output token other than A at position T}” as 1 to train the auxiliary classifier. Following the neuron identification strategy, there are about 15\%$\sim$25\% neurons belonging to $S_{store,A}$. In addition, we discover an interesting fact that neuron index in $S_{store,A}$ for t=1, t=2, ..., until t=T-1 are almost the same and the neuron values remain largely unchanged. To visualize the situation, we plot the values of top ten neurons in $S_{store,A,t=T-1}$ (they also appears at almost other steps $t < T - 1$) in Figure \ref{store_trend}. One can discover that many of them keeping unchanged from $t = -1$ (\emph{Token} signal first appears in the encoder) to $t = T - 1 = 5$ (one step before the model outputs the token). In addition, we also compare the storing neuron for top ten common tokens in Figure \ref{S_store}. We plot the PCA diagram for all storing neurons with the same dimension reduction transformation in each sub-figure and it also shows that storing neurons for different tokens truly stay at their own positions from $t = -1$ to $T − 1$.
The last step for this question is to verify two things. Firstly,  $S_{store,A}$ is necessary for model to output the token. Therefore, we replace the values of $S_{store,A}$ at t = T − 1 with zero, and found the token accuracy drops significantly although about 80\% of neurons remaining the same. Secondly, we need to verify that model use the same neuron index and even the same value to store one important information passing through the entire encoder and decoder. Hence, we then replace values of the storing neurons by their previous states, and find that accuracy remains respectfully high. The average accuracy of two datasets is shown in Table \ref{table verification}.




\begin{figure}[h]
    \begin{center}
    
    \begin{minipage}[b]{0.43\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figures/store.png}
        \caption{$S_{store,tok}$ values from encoder to decoder. We plot the hidden states of ten $S_{store,tok=i}$ neurons with \emph{Pos.} = 5. Their values remain unchanged from t = \emph{Token} until 4, when it is ready to trigger $S_{fc,tok}$.}
        \label{store_trend}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.53\textwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{figures/word_encoder_cd_with_label_2.png}
         \caption{Mean values of $S_{cd}$ through time step with different assigned $T$. (Some neurons are flipped through all steps for visualization convenience.) 
         The values with different T scatter when \emph{Pos.} is provided and reach the highest value in order according to T.}
         \label{cd}
    \end{minipage}%
    \end{center}
    
    \label{POS_10}
\end{figure}

\subsection{How does the model use $position$ signal to know when to output?}
To answer this question, we turn to take all samples that output A at any T, and give the classification label as “T - t”. For example, the hidden state at step t = 3 with T = 5 and t = 4 with T = 6 share the same label = 2, because both of them have two steps left to output the token. Applying the same strategy, there are about 20\% neurons belongs to $S_{cd,A}$ after filtering. Then, the next question is: how does $S_{cd,A}$ count? %Similarly, we plot the real values of the hidden state of the top ten counting neurons in Figure \ref{}. 
We first find out that the values of the counting neurons increase or decrease gradually through time step. Next, we flip (multiply with -1) all neurons whose values are decreasing ($S_{cd,A,t=T-2} < S_{cd,A,t=1}$), then take the average of all counting neurons. The result is shown as Figure \ref{cd}. Each different colored line represents a different target position T. When the Position signal appears at t = 0 in the encoder, the values of counting neurons start to spread out. Then, in the next few steps, counting neurons jointly behave as a incremental function that gradually reaches the optimal at t = T - 1. 
The last step is to verify $S_{cd,A}$ that it can indicates how many steps it should takes to reach the target positioning. 
We replace the value of $S_ {cd, A} $ at t with the value of t − 1 (the previous stage), and calculate how much data will output the assigned token for one step delay.
We show the results of t = 2, 3, and 4 in table \ref{table verification}. The average accuracy of all common tokens is high reveals that the $S_{cd,A}$ neuron indeed performs as expected.


\begin{table}[h!]
	\centering
	\label{table verification}
	\caption{Verification on $S_{trig,tok}$. For each token with $T$ = 6, we substitute the value $S_{trig,tok}$ at $t = T-1$ to 1 to 4 steps earlier and verify that the token can be outputted also earlier. }
	
	\begin{tabular}{c|cccc|cc|ccc}
		\toprule
		Neuron set & \multicolumn{4}{c|}{Trigger} & \multicolumn{2}{c|}{Store} & \multicolumn{3}{c}{Count down}\\
		Accuracy (\%) & 1 step & 2 steps & 3 steps & 4 steps & Zero & Previous & t = 2 & t = 3 & t = 4 \\
		\midrule
		Lyrics Freak & 99.8 & 96.4 & 91.2 & 84.1  & 10.7 & 87.9 & 99.9 & 99.9 & 99.3 \\
		Gutenberg & 94.2 & 93.0 & 91.4 & 90.4 & 20.0 & 83.3 & 98.9 & 99.3 & 99.5 \\
		Ideal situation & high & high & high & high & low & high & high & high & high\\
	\bottomrule
	\end{tabular}
	
	\label{S_trigger}
\end{table}


\subsection{How does the model combine $token$ and $position$ information to output? }

To answer the third question, we need to further introduce the last two important neuron sets, triggering and outputting neuron. 

$\boldsymbol{S_{trig,A}}$: $S_{trig,A}$ is the neuron set triggering the model to output the token exactly at the next step. To train the auxiliary classifier, we label $h_{t=T−1}$ as 0 and $h_t$ with every t < T −1 as 1, for each token A and position T. There are about 15\% ∼ 25\% neurons belonging to $S_{trig,A}$ after filtering. The next step is to verify $S_{trig,A}$. We replace the value of $S_{trig,A}$ at $h_{t=T-1}$ to any time t, with $0 <= t < T$, and check whether the model outputs the target token exactly at the next step. The table \ref{table verification} shows the average accuracy that we perform experiments on 50 common tokens and original target position = 6 on each dataset. We replace the value of trigger neuron at t = 5 (since $T - 1 = 6 - 1 = 5$) to t = 1, 2, 3 and 4 respectively, and the model outputs the tokens immediately at these four steps with very high probability. Actually, $S_{trig,A}$ can also be seen as the last step of the counting neuron.

$\boldsymbol{S_{out,A}}$: The outputting neuron is a set of neuron causing the fully connected layer to output the target token at t = T. Back to the model structure in Figure \ref{structure}, when the model needs to output token A at position T, the probability of outputting token A should be the largest. Besides, this probability is proportional to $h_{t=T} W_{tok=A}$. However, only a small sets (about 20\%) of neuron in $h_{t=T}$ play most of the effects to influence the values of $h_{t=T} W_{A}$ and they tends to close to -1 or +1 because the range of GRU hidden states is from -1 to +1. We define this small set of neurons as outputting neuron.
To find out outputting neuron, one can apply the strategy described previously, or simply find the neurons with the largest $h_{t=T} W_{A}$, as $W_{A}$ represents the learned fully connected weights connected to target token A.
The verification process goes as below: we zero-out the values of $S_{out,A}$ and remain other 80\% neurons on $h_{t=T}$ before feeding into the fully connected layer, and the mean accuracy of token positioning dropped to 0.0\%. On the other hand, we keep the values of neurons belongs to $S_{out,A}$ and zero-out others 80\% of neurons. The accuracy remains as high as 99.9\%. This indicate that $S_{out,A}$ in $h_{t=T}$ is critical to the output of the token.

%\textbf{Neuron interaction:} 
% 把之前的section 5 移一小段進來解釋第三個問題
% \section{Appendix}
\textbf{Interaction between Functional Neurons and Gates inside GRU}

After realizing the validity of four functional neurons, we go deep into the formulation of GRU, including each gate and its corresponding weight.
% After the model encoded the word information with storing neuron and the position information with counting neuron, it raised another question to  solve: what is the interaction between storing and counting neuron to trigger model output the right word at the right time-step ? 
In the following, we combine the mathematical and the empirical perspective to investigate the relationship between functional neurons and gates. 

%\newpage

Recall the mathematical formulation of GRU cell:

% \begin{small}
\begin{equation*}
% \begin{aligned}
GRU\begin{cases}
    &z_t = \sigma(W_{z}x_t + U_{z}h_{t-1} + b_z)  \\
    &r_t = \sigma(W_{r}x_t + U_{r}h_{t-1} + b_r) \\
    &\widetilde{h_t} = \text{tanh}(W_{h}x_t + U_{h}(r_t \odot h_{t-1}) + b_h)  \\ 
    &h_t = z_t \odot h_{t-1} + (1 - z_t) \odot \widetilde{h}_t\\
    \end{cases} \quad
GRU^{'}\begin{cases}
    &z_t = \sigma(U_{z}h_{t-1} + b_z)  \\
    &r_t = \sigma(U_{r}h_{t-1} + b_r) \\
    &\widetilde{h_t} = \text{tanh}(U_{h}(r_t \odot h_{t-1}) + b_h)  \\ 
    &h_t = z_t \odot h_{t-1} + (1 - z_t) \odot \widetilde{h}_t
    \end{cases}
% \begin{aligned}
%     &z_t = \sigma(W_{z}x_t + U_{z}h_{t-1} + b_z)  \\
%     &r_t = \sigma(W_{r}x_t + U_{r}h_{t-1} + b_r) \\
%     &\widetilde{h_t} = \text{tanh}(W_{h}x_t + U_{h}(r_t \odot h_{t-1}) + b_h)  \\ 
%     &h_t = z_t \odot h_{t-1} + (1 - z_t) \odot \widetilde{h}_t\\
% \end{aligned}
\label{GRU_Formula}
\end{equation*}
% \end{small}
% \caption{The original formulation of GRU and its simplified version}


with $z_t, r_t, h_t, \widetilde{h}_t$ as the \emph{update gate}, \emph{reset gate}, \emph{activation}, and \emph{candidate activation}.


One of the side-findings reveals that, as an GRU decoder takes the previous state $h_{t-1}$ and the produced token  $x_{t}$ as two inputs, we found that $x_{t}$ contribute almost nothing to the token-positioning task. We confirm this hypothesis by simply replacing $x_{t}$ with a random token and the accuracy remains 98.0\%. Since the random replacement experiment shows that $x_t$ has very few influence on $z_t, r_t, h_t$ that can be neglected, we simplify the formulation of GRU cell and noted as $GRU^{'}$. Then we can simply view the operation inside the $\sigma(\cdot)$ function as a linear transformation of $h_{t-1}$ to $z_t, r_t$ or $h_t$. Therefore, the weight $U_z, U_r, U_h$ are indeed the feature importance. 
Based on these simplifications, we can visualize the neuron interaction as in Figure \ref{interaction}.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/appendix_trig_vis.png}
    \caption{Visualization of neurons interaction. }
    \label{interaction}
\end{figure}

% \begin{small}
% \begin{equation}
% \begin{aligned}
%     &z_t = \sigma(U_{z}h_{t-1} + b_z)  \\
%     &r_t = \sigma(U_{r}h_{t-1} + b_r) \\
%     &\widetilde{h_t} = \text{tanh}(U_{h}(r_t \odot h_{t-1}) + b_h)  \\ 
%     &h_t = z_t \odot h_{t-1} + (1 - z_t) \odot \widetilde{h}_t
% \end{aligned}
% \label{GRU}
% \end{equation}
% \end{small}

In order to verify our hypothesis that triggering neurons unblock the storing neurons to affect the outputting neurons, we observe the transition weight in $U_z, U_r, U_h$ from triggering neurons to storing neurons or outputting neurons. The higher the absolute value of transition weight, the more important it is. Following the formulation above,  for \emph{z gate}, the transition weight from triggering neuron to outputting neurons should be low in order to update the neuron value in $h_{t-1}$ (in Fig. \ref{interaction}(a)), and for the \emph{r gate}, the transition weight from trigger neuron to storing neuron should be high in order to make $h_{t-1}$ effective to $\widetilde{h_t}$  or it will be masked.(in Fig. \ref{interaction}(b))  After the value in each gate are determined, the transition weight in $U_h$ should be extreme value in order to trigger the outputting neurons to reach extreme value as well.(in Fig. \ref{interaction}(c)) Additionally, we apply integrated gradient to check the impact from triggering neuron to outputting neurons, which shows the same result as directly analyzing the inner operation of GRU cell. Statistics are listed in Figure X and Table X.





% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{ccccc}
% 		\toprule
% 		Neurons set & Z gate & R gate & H gate \\
% 		\midrule
% 		$h_{T-1, store}$ & 7.9E-3 & 7.3E-3 & 6.7E-3\\
% 		$h_{T-1, trig}$ & 1.3E-2 & 9.8E-3 & 1.6E-3 \\
% 		Whole $h_{T-1}$ & 4.0E-3 & 5.1E-3  & 2.4E-3\\
% 		\bottomrule
		
% 	\end{tabular}
	
% 	\caption{Different $S_{Imp}$ importance through different gates by calculating integrated gradient score. The first and second columns show that $h_{T-1, trig}$ is the most important through z and r gate, whereas the third column shows that $h_{T-1, store}$ is the most important through h gate.}
% 	\label{IG_score}
% \end{table}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/appendix_z_impact.png}
%   \caption{Impact of triggering neurons to decrease \emph{z gate} value of outputting neurons. X-axis are sixteen $S_{fc,tok}$ neurons. Y-axis represents the impact from $h_{T-1, trig}$ (blue bars) and other neurons (red bars). Most blue bars have obvious negative values and it implies that it is $h_{T-1, trig}$ to increase $z_{T, fc}$.}
%   \label{z_impact}
% \end{figure}




\begin{figure}[h]
    \begin{center}
    
    \begin{minipage}[b]{0.43\textwidth}
        \centering
        	\begin{tabular}{ccccc}
    		\toprule
    		Neurons set & Z gate & R gate & H gate \\
    		\midrule
    		$h_{T-1, store}$ & 7.9E-3 & 7.3E-3 & 6.7E-3\\
    		$h_{T-1, trig}$ & 1.3E-2 & 9.8E-3 & 1.6E-3 \\
    		Whole $h_{T-1}$ & 4.0E-3 & 5.1E-3  & 2.4E-3\\
    		\bottomrule
        		
        	\end{tabular}
        	
        	\caption{Different $S_{Imp}$ importance through different gates by calculating integrated gradient score. The first and second columns show that $h_{T-1, trig}$ is the most important through z and r gate, whereas the third column shows that $h_{T-1, store}$ is the most important through h gate.}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.53\textwidth}
         \centering
         \includegraphics[width=0.6\textwidth]{figures/appendix_z_impact.png}
          \caption{Impact of triggering neurons to decrease \emph{z gate} value of outputting neurons. X-axis are sixteen $S_{fc,tok}$ neurons. Y-axis represents the impact from $h_{T-1, trig}$ (blue bars) and other neurons (red bars). Most blue bars have obvious negative values and it implies that it is $h_{T-1, trig}$ to increase $z_{T, fc}$.}
          \label{z_impact}
        
    \end{minipage}%
    \end{center}
    
    \label{POS_10}
\end{figure}

\end{comment}










